A new class of curves of rational B-spline type

A new class of rational parametrization has been developed and it was used to generate a new family of rational functions B-splines $\displaystyle{{\left({}^{\alpha}{\mathbf B}_{i}^{k} \right)}_{i=0}^{k}}$ which depends on an index $\alpha \in (-\infty,0)\cup (1,+\infty)$. This family of functions verifies, among other things, the properties of positivity, of partition of the unit and, for a given degree k, constitutes a true basis approximation of continuous functions. We loose, however, the regularity classical optimal linked to the multiplicity of nodes, which we recover in the asymptotic case, when $\alpha \longrightarrow \infty$. The associated \mbox{B-splines} curves verify the traditional properties particularly that of a convex hull and we see a certain "conjugated symmetry" related to $\alpha$. The case of open knot vectors without an inner node leads to a new family of rational Bezier curves that will be separately, object of in-depth analysis.

==> SortieBspline5en.tex <==
%Base Bspline de degre 2 avec un vecteur noeud a un noeud interieur double
\newpage
B-spline basis of degree 2 and its derivative
for the knot vector\\
$U=\left( x_{0},x_{0}, x_{0}, x_{1}, x_{1}, x_{2}, x_{2}, x_{2} \right)$

$$
\Bspline{i}{2}{\alpha} (t)=
\left\lbrace
\begin{array}{ll}
{{\left(\alpha-1\right)^2\,\left({\it x_1}-t\right)^
 2}\over{\left(\alpha\,{\it x_1}-{\it x_1}-\alpha\,{\it x_0}+t\right)
 ^2}}
&\textrm{if } i=0 \textrm{ and } t\in [x_{0}\, , \, x_{1}[\\ 
-{{2\,\left(\alpha-1\right)\,\alpha\,\left({\it x_0}-t
 \right)\,\left({\it x_1}-t\right)}\over{\left(\alpha\,{\it x_1}-
 {\it x_1}-\alpha\,{\it x_0}+t\right)^2}}
&\textrm{if } i=1 \textrm{ and } t\in [x_{0}\, , \, x_{1}[\\ 
{{\alpha^2\,\left(
 {\it x_0}-t\right)^2}\over{\left(\alpha\,{\it x_1}-{\it x_1}-\alpha
 \,{\it x_0}+t\right)^2}}
&\textrm{if } i=2 \textrm{ and } t\in [x_{0}\, , \, x_{1}[\\ 
{{\left(\alpha-1\right)^2\,\left(
 {\it x_2}-t\right)^2}\over{\left(\alpha\,{\it x_2}-{\it x_2}-\alpha
 \,{\it x_1}+t\right)^2}}
&\textrm{if } i=2 \textrm{ and } t\in [x_{1}\, , \, x_{2}[\\ 
-{{2\,\left(\alpha-1\right)\,\alpha\,
 \left({\it x_1}-t\right)\,\left({\it x_2}-t\right)}\over{\left(
 \alpha\,{\it x_2}-{\it x_2}-\alpha\,{\it x_1}+t\right)^2}}
&\textrm{if } i=3 \textrm{ and } t\in [x_{1}\, , \, x_{2}[\\ 
{{
 \alpha^2\,\left({\it x_1}-t\right)^2}\over{\left(\alpha\,{\it x_2}-
 {\it x_2}-\alpha\,{\it x_1}+t\right)^2}}
&\textrm{if } i=4 \textrm{ and } t\in [x_{1}\, , \, x_{2}[\\ 
0 
&\textrm{otherwise } \\ 
\end{array}
\right.
$$

% Derivee
$$
\frac{d}{dt}\Bspline{i}{2}{\alpha} (t)=
\left\lbrace
\begin{array}{ll}
-{{2\,\left(\alpha-1\right)^2\,\alpha\,\left(
 {\it x_1}-t\right)\,\left({\it x_1}-{\it x_0}\right)}\over{\left(
 \alpha\,{\it x_1}-{\it x_1}-\alpha\,{\it x_0}+t\right)^3}}
&\textrm{if } i=0 \textrm{ and } t\in [x_{0}\, , \, x_{1}[\\ 
{{2
 \,\left(\alpha-1\right)\,\alpha\,\left({\it x_1}-{\it x_0}\right)\,
 \left(\alpha\,{\it x_1}-{\it x_1}+\alpha\,{\it x_0}-2\,\alpha\,t+t
 \right)}\over{\left(\alpha\,{\it x_1}-{\it x_1}-\alpha\,{\it x_0}+t
 \right)^3}}
&\textrm{if } i=1 \textrm{ and } t\in [x_{0}\, , \, x_{1}[\\ 
-{{2\,\left(\alpha-1\right)\,\alpha^2\,\left(
 {\it x_0}-t\right)\,\left({\it x_1}-{\it x_0}\right)}\over{\left(
 \alpha\,{\it x_1}-{\it x_1}-\alpha\,{\it x_0}+t\right)^3}}
&\textrm{if } i=2 \textrm{ and } t\in [x_{0}\, , \, x_{1}[\\ 
-{{
 2\,\left(\alpha-1\right)^2\,\alpha\,\left({\it x_2}-t\right)\,\left(
 {\it x_2}-{\it x_1}\right)}\over{\left(\alpha\,{\it x_2}-{\it x_2}-
 \alpha\,{\it x_1}+t\right)^3}}
 &\textrm{if } i=2 \textrm{ and } t\in [x_{1}\, , \, x_{2}[\\ 
 {{2\,\left(\alpha-1\right)\,
 \alpha\,\left({\it x_2}-{\it x_1}\right)\,\left(\alpha\,{\it x_2}-
 {\it x_2}+\alpha\,{\it x_1}-2\,\alpha\,t+t\right)}\over{\left(\alpha
 \,{\it x_2}-{\it x_2}-\alpha\,{\it x_1}+t\right)^3}}
&\textrm{if } i=3 \textrm{ and } t\in [x_{1}\, , \, x_{2}[\\ 
-{{2\,
 \left(\alpha-1\right)\,\alpha^2\,\left({\it x_1}-t\right)\,\left(
 {\it x_2}-{\it x_1}\right)}\over{\left(\alpha\,{\it x_2}-{\it x_2}-
 \alpha\,{\it x_1}+t\right)^3}}
&\textrm{if } i=4 \textrm{ and } t\in [x_{1}\, , \, x_{2}[\\ 
0 
&\textrm{otherwise } \\ 
\end{array}
\right.
$$

% limite en x1
$$
\lim_{t\to x_{1}}\Bspline{i}{2}{\alpha} (t)=
\left\lbrace
\begin{array}{ll}
1
&\textrm{if } i=2 \textrm{ and } t\in [x_{0}\, , \, x_{1}[\\ 
1
&\textrm{if } i=2 \textrm{ and } t\in [x_{1}\, , \, x_{2}[\\ 
0
&\textrm{otherwise } \\ 
\end{array}
\right.
$$

%limite de la derive e x1
$$
\lim_{t\to x_{1}}\frac{d}{dt}\Bspline{i}{2}{\alpha} (t)=
\left\lbrace
\begin{array}{ll}
-{{2\,\left(\alpha-1\right)}\over{\alpha\,
 \left({\it x_1}-{\it x_0}\right)}}
&\textrm{if } i=1 \textrm{ and } t\in [x_{0}\, , \, x_{1}[\\ 
{{2\,\left(\alpha-1\right)
 }\over{\alpha\,\left({\it x_1}-{\it x_0}\right)}}
&\textrm{if } i=2 \textrm{ and } t\in [x_{0}\, , \, x_{1}[\\ 
-{{2\,\alpha
 }\over{\left(\alpha-1\right)\,\left({\it x_2}-{\it x_1}\right)}}
&\textrm{if } i=2 \textrm{ and } t\in [x_{1}\, , \, x_{2}[\\ 
 {{2\,\alpha}\over{\left(\alpha-1\right)\,\left({\it x_2}-
 {\it x_1}\right)}}
&\textrm{if } i=3 \textrm{ and } t\in [x_{1}\, , \, x_{2}[\\ 
0 
&\textrm{otherwise } \\ 
\end{array}
\right.
$$


